Fine-grained Analysis of Sentence Embeddings Using Auxiliary Prediction Tasks

There is a lot of research interest in encoding variable length sentences into fixed length vectors, in a way that preserves the sentence meanings. Two common methods include representations based on averaging word vectors, and representations based on the hidden states of recurrent neural networks such as LSTMs. The sentence vectors are used as features for subsequent machine learning tasks or for pre-training in the context of deep learning. However, not much is known about the properties that are encoded in these sentence representations and about the language information they capture. We propose a framework that facilitates better understanding of the encoded representations. We define prediction tasks around isolated aspects of sentence structure (namely sentence length, word content, and word order), and score representations by the ability to train a classifier to solve each prediction task when using the representation as input. We demonstrate the potential contribution of the approach by analyzing different sentence representation mechanisms. The analysis sheds light on the relative strengths of different sentence embedding methods with respect to these low level prediction tasks, and on the effect of the encoded vector's dimensionality on the resulting representations.

==> experimental_setup.tex <==
\subsection{Data}
All the sentences in our datasets are taken from Wikipedia dump 2012. We use NLTK~\citep{bird2006nltk} for tokenization. Sentence lengths are constrained to be between 5 and 70 words.

%\hl{The sentences used for training the sentence embeddings are distinct from those
%used for creating the auxiliary prediction tasks.}

%\subsection{Setup for the three tests}
%Table~\ref{tab:tests-data} provides some statistics for the datasets used for all our tests. Note that our approach allows us to easily create large datasets.

%For the content and order tests there are one positive and one negative examples per sentence, so the total number of examples is twice the number of sentences. For the length test, we bin every four consecutive lengths (5-8, 9-12, etc.) and collapse all lengths greater than 34 words. This makes for a balanced dataset.  
%We use the following length bins: $\{5-8, 9-12, 13-16, 17-20, 21-25, 26-29, 30-33, 34-70 \}$. 

%\begin{table}[t]
%\small
%\centering
%\begin{tabular}{| c | c | c | c |}
%\hline  & \bf Train & \bf Validation & \bf Test \\ 
%\hline
% \# sentences & 150k & 25k & 25k \\ 
% \hline
%\end{tabular}
%\caption{\label{tab:tests-data} Dataset sizes for the main tests.}
%\end{table}

%Regarding our testing method, we implemented one hidden layer neural network with ReLU \cite{nair2010rectified,glorot2011deep} as an activation function. We use one dropout layer with 0.8 dropout rate and softmax layer on top of the network. The size of the hidden layer is the same as the size of the input layer in all the tests. We optimize all the tests with AdaGrad \cite{duchi2011adaptive} using 0.01 learning rate. In all the tests we use 150,000 sentences for training, 25,000 sentences for test and 25,000 sentences for validation. All the sentences contains between 5 to 70 words each, and were taken from wikipedia corpus. We stopped training the tests after 5 epochs with no loss improvement on the validation set.

\subsection{Setup for Sentence Representation Models}
The auto-encoder and CBOW models are trained on 1 million sentences. 
%All sentence embedding models, with the exception of skip-thought, were trained on 1 million sentences.

For the bag-of-words model, we train Skip-gram word vectors~\citep{mikolov2013efficient}, with hierarchical-softmax and a window size of 5 words, using the Gensim implementation.\footnote{\url{https://radimrehurek.com/gensim}}. We control for the embedding size $k$ and train word vectors of sizes $k \in \{100,300,500,750,1000\} $.

For the encoder-decoder models, we use an in-house implementation using the Torch7 tookit~\citep{collobert2011torch7}. The decoder is trained as a language model, attempting to predict the correct word at each time step using a negative-log-likelihood objective (cross-entropy loss over the softmax layer).
%For training the encoder-decoder models, we consider two different loss functions. First, we pass the decoder outputs at each time-step to a Softmax layer, and compute the posterior probability of all the words in the vocabulary. In this case we optimize the negative log-likelihood. Note that the size of the Softmax layer is $d\times |V|$, where $|V|$ is the vocabulary size, which can be quite large. To  save computation, we remove the Softmax layer and replace the log-likelihood loss with a cosine similarity loss over the predicted and true word representations for each word in the sentence. We refer to this model as a Regression model.

We always use the same dimension for word and sentence representations (i.e.
$d=k$), and train models of sizes  $k \in \{100,300,500,750,1000\}$. The models
are optimized using AdaGrad, whose learning rate is tuned on a dedicated
validation set. Other settings are similar to previous work on
sequence-to-sequence learning~\citep{sutskever2014sequence,li2015hierarchical},
including reversing input sentences and clipping gradients. Word vectors are
initialized to random values. % when optimizing the negative log-likelihood,\footnote{We
%experimented with pre-trained Skip-gram word vectors and have not noted a
%significant difference in performance.}.% and pre-trained with Skip-gram when optimizing the cosine-similarity.
Encoder-Decoder models are trained on a single GPU, with minibatches of 32 sentences; training takes approximately 10 days and is stopped after 5 epochs with no loss improvement on a validation set. We use the LSTM implementation in \citet{leonard2015rnn}.

%For some experiments we replace the LSTM encoder with a Simple-RNN \cite{elman} encoder.

For all the encoder-decoder models we compute BLEU scores \citep{papineni2002bleu}, a popular machine translation evaluation metric that is also used to evaluate auto-encoder models \citep{li2015hierarchical}. As BLEU score measures how well the original sentence is re-created, it can be thought of as a proxy for the quality of the encoded representation. We will compare it with the performance of the models on our three main tests.  

For the skip-thought vectors, we use the pre-trained models, with the recommended embedding size of 4800. 
%Skip-Thoughts require a corpus with consecutive sentences, while our dataset contains random sentences from Wikipedia with no constraint of being from the same article.



==> results_bu.tex <==
In this section we provide a detailed description of our experimental results along with their analysis.

%%% CONTENT %%%
\subsection{Content Experiments}
Recall, our goal is to find out whether the sentence representation contains information about the identity of the words in it. In other words, we would like to assess the relation between the sentence and word representations.

We begin by presenting the results for the encoder-decoder model using different LSTM sizes, Table~\ref{acc_lstm_size} second column presents that results.

%\begin{table}[H]
%\small
%\centering
%\begin{tabular}{| c | c | c | c |}
%\hline \bf Rep. & \bf Random & \bf Order of & \bf Sentence \\ 
% \bf Size & \bf Word (acc\%)& \bf Word (acc\%)& \bf Length (acc\%)\\  \hline
%100 & 70 & 78 & 50 \\
%300 & 76 & 85 & 82 \\
%500 & 76 & 88 & \textbf{87} \\
%750 & \textbf{80} & 88 & 80 \\
%1000 & 75 & \textbf{91} & \textbf{87} \\
%\hline
%\end{tabular}
%\caption{\label{acc_lstm_size} Test accuracy for different LSTM sizes.}
%\end{table}

% \begin{table}[H]
% \small
% \centering
% \begin{tabular}{| c | c |}
% \hline \bf Representation Size & \bf Accuracy \\ \hline
% 100 & 70\% \\
% 300 & 76\% \\
% 500 & 76\% \\
% 750 & 80\% \\
% 1000 & 75\% \\
% \hline
% \end{tabular}
% \caption{\label{rand_lstm_size} Random word accuracy for different LSTM sizes.}
% \end{table}

We can see from Table~\ref{} that the LSTMs are capturing information about the identity of the words. An interesting property to note is the drop of the accuracy once we reach representation size of 1000. This drop is in contrast to the BLEU score we get from the full encoder-decoder model. Figure~\ref{fig:rand_bleu_lstm_size} visualize the random accuracy against the BLEU score for all of the LSTM with different sizes.

Next, we wanted to inspect the effect of using different encoders for the sentence. We still use the encoder-decoder architecture but only changing the encoder type. We compare the results of LSTM, Bi-Directional-LSTM (BI-LSTM), RNN and CNN all of which with size 1000. The results are presented in Table~\ref{acc_different_encoders} in the second column.
%We choose size 1000 since it provides the best results from the previous test.
We can see that it is much harder to find the relation between word and sentence representations when encoding the sentence using CNN and RNN. While in many tasks BI-LSTM preforms better then standard LSTM, here it makes it a little bit harder to find the relation.

%\begin{table}[H]
%\small
%\centering
%\begin{tabular}{| c | c | c | c |}
%\hline \bf Encoder & \bf Random & \bf Order of & \bf Sentence \\ 
% \bf Type & \bf Word & \bf Word & \bf Length \\  \hline
%LSTM & \textbf{75} & \textbf{91} & 87 \\
%BI-LSTM & 70 & 50 & \textbf{97} \\
%RNN & 60 & 50 & 13 \\
%CNN & 59 & 62 & 13 \\
%\hline
%\end{tabular}
%\caption{\label{acc_different_encoders} Test accuracy for different encoder types, all of the model use size 1000 as their representation size.}
%\end{table}

%\begin{table} [H]
%\end{table}

% \begin{table} [H]
% \small
% \centering
% \begin{tabular}{| c | c |}
% \hline \bf Encoder Type & \bf Accuracy \\ \hline
% LSTM & 75\% \\
% BI-LSTM & 70\% \\
% RNN & 60\% \\
% CNN & 59\% \\
% \hline
% \end{tabular}
% \caption{\label{rand_different_encoders} Word containment accuracy for different encoder types, all of the model use size 1000 as their representation size.}
% \end{table}
Lastly, we present the results of different models, CBOW with different embed size, Skip-Thoughts model with representation size if 4800 as recommended in the paper, and encoder-decoder using LSTM of size 750.

%\begin{table} [H]
%\small
%\centering
%\begin{tabular}{| c | c |}
%\hline \bf Model Type & \bf Accuracy (\%) \\ \hline
%Skip-Thoughts & 80 \\
%LSTM & 80 \\
%CBOW (100) & 83 \\
%CBOW (300) & 88 \\
%CBOW (500) & 60 \\
%CBOW (750) & 60 \\
%CBOW (1000) & 60 \\
%\hline
%\end{tabular}
%\caption{\label{rand_different_models} Random word accuracy for different models.}
%\end{table}

We can see from Table~\ref{rand_different_models} that all the models were managed to find relation between word and sentence representations. Skip-Thoughts reached the same accuracy as the standard encoder-decoder although was not trained on the same corpus. The results of CBOW with embedding size of 300 outperforms all the other models, although CBOW with embed size of 100 also provides good results. \hl{Interesting to notice how the CBOW accuracy drops dramatically while increasing the embedding size.}

\begin{figure}[!h]
  \caption{\label{fig:content_bleu} BLEU score against content word experiment for all the models.}
  \centering
    \includegraphics[width=0.5\textwidth]{img/random_word.png}
\end{figure}

%%% ORDER %%%
\subsection{Order Experiments}
In the order experiment our goal is to find out whether the sentence representation contains information about the order of the words that were encoded into it, i.e what word was encoded first.

% \begin{table}[H]
% \small
% \centering
% \begin{tabular}{| c | c |}
% \hline \bf Representation Size & \bf Accuracy \\ \hline
% 100 & 78\% \\
% 300 & 85\% \\
% 500 & 88\% \\
% 750 & 88\% \\
% 1000 & 91\% \\
% \hline
% \end{tabular}
% \caption{\label{order_lstm_size} Words order accuracy for different LSTM sizes.}
% \end{table}

It seems from Table~\ref{acc_lstm_size} column three that the encoder-decoder model using LSTMs produces representations that contains information about the words order. However, there is not much of a difference between the LSTM of size 500, 750 and 1000. When considering the BLEU score of those models the question that is being raised is: does the encoder encodes more information into the representation or is it just the decoder that got better?

\begin{figure}[!h]
  \caption{\label{fig:order_bleu_lstm_size} BLEU score against words order accuracy with respect to different LSTM sizes.}
  \centering
    \includegraphics[width=0.5\textwidth]{img/LSTMsizeVSacc_bleu.jpg}
\end{figure}

%When considering different encoders, we see that it is much harder to find the relation between word and sentence representations when encoding the sentence using CNN and RNN. While in many tasks BI-LSTM preforms better then standard LSTM, here it makes it a little bit harder to find the relation.
%
%\begin{table} [H]
%\small
%\centering
%\begin{tabular}{| c | c |}
%\hline \bf Encoder Type & \bf Accuracy \\ \hline
%LSTM & 91\% \\
%BI-LSTM & 50\% \\
%RNN & 50\% \\
%CNN & 62\% \\
%\hline
%\end{tabular}
%\caption{\label{rand_different_encoders} Word containment accuracy for different encoder types, all of the model use size 1000 as their representation size.}
%\end{table}

When considering different models we can see from Table~\ref{order_different_models} that the Skip-Thoughts representations do contains order information, its performance is as good as the standard encoder-decoder although not trained on the same corpus. The more interesting case is the one with CBOW models. Somehow, it manage to reach 70\% accuracy at the order task, (the data set is balanced so majority classification is 50\%) although not contains any information about the order of the words. One way to explain this phenomena is by considering language statistics, i.e if word $w$ appears before word $u$ most of the times than there is no need to encode this information into the representation, we can infer this only by following language statistics.

\begin{table} [H]
\small
\centering
\begin{tabular}{| c | c| c |}
\hline \bf Model Type & \bf Accuracy (\%) \\ \hline
Skip-Thoughts & 91 \\
LSTM & 91 \\
CBOW (100) & 70 \\
CBOW (300) & 70 \\
CBOW (500) & 66 \\
CBOW (750) & 66 \\
CBOW (1000) & 66 \\
\hline
\end{tabular}
\caption{\label{order_different_models} Words order accuracy for different models.}
\end{table}

To account for this, we rerun the same test but this time we dropped the sentence representation. In other words, we fed the network two word representations and ask the network what word come first in the sentence. This way, we can better understand what is the role of language and if the presence of all the words in the sentence (i.e sentence representation) helps when classifying what word came first.

\begin{table} [H]
\small
\centering
\begin{tabular}{| c | c| c | c |}
\hline \bf  & \bf LSTM & \bf CBOW & \bf Skip-Thoughts \\ \hline
100 & 67 & 67 & - \\
300 & 67 & 68 & -\\
500 & 67 & 65 & -\\
750 & 67 & 64 & -\\
1000 & 65 & 64 & -\\
1280 & - & - & ? \\
\hline
\end{tabular}
\caption{\label{order_no_sentence} Words order accuracy without sentence representation for all the models (results are in percentage).}
\end{table}

We can see from Table~\ref{order_no_sentence} that the difference between including and removing the sentence representation is minor in that test, which means that the classifier probably ignores the sentence representation and did not extract any relevant information from it.

\begin{figure}[!h]
  \caption{\label{fig:order_vs_word_distance} Add caption.}
  \centering
    \includegraphics[width=0.5\textwidth]{img/order_vs_distance.png}
\end{figure}
\mycomment{Maybe add something like that plot here?}

%%% LENGTH %%%
\subsection{Length Experiments}
The last test we describe is related to the sentence length. In that test we would like to find out whether the sentence representation contains information about the number of words that were encoded into it.
The fourth column in Table~\ref{acc_lstm_size} present the results for the encoder-decoder model using different sizes of LSTMs.

% \begin{table}[H]
% \small
% \centering
% \begin{tabular}{| c | c |}
% \hline \bf Representation Size & \bf Accuracy \\ \hline
% 100 & 50\% \\
% 300 & 82\% \\
% 500 & 87\% \\
% 750 & 80\% \\
% 1000 & 87\% \\
% \hline
% \end{tabular}
% \caption{\label{len_lstm_size} Sentence length accuracy for different LSTM sizes.}
% \end{table}
Table~\ref{} suggests that the representations generated using LSTMs captures a lot of information on the sentence length, even when we use representation size of 100 we reach 50\% accuracy rate which is not bad when considering the fact that our baseline in this task is$\sim$20\%.

% \begin{table} [H]
% \small
% \centering
% \begin{tabular}{| c | c |}
% \hline \bf Encoder Type & \bf Accuracy \\ \hline
% LSTM & 87\% \\
% BI-LSTM & 96\% \\
% RNN & 13\% \\
% CNN & 13\% \\
% \hline
% \end{tabular}
% \caption{\label{different_encoders} Sentence length accuracy for different encoder types, all of the model use size 1000 as their representation size.}
% \end{table}

When considering different encoders, Table~\ref{acc_different_encoders} fourth column, you can see that Bi-LSTM outperforms the basic LSTM but the performance of the SimpleRNN and the CNN at this task is poor.

\begin{table} [H]
\small
\centering
\begin{tabular}{| c | c |}
\hline \bf Model Type & \bf Accuracy (\%) \\ \hline
CBOW & 50 \\
Skip-Thoughts & 82 \\
LSTM & 87 \\
\hline
\end{tabular}
\caption{\label{sen_len_different_models} Sentence length accuracy for different models.}
\end{table}
Lastly, Table~\ref{sen_len_different_models} present the accuracy of the different models.
We can see that the Skip-Thoughts model is slightly worse than the standard encoder-decoder, however it was trained on a different corpus, and again the CBOW model is surprisingly not bad. As a result we come up with the question: Does the CBOW works good because of the language properties or because of some other reason?

\begin{table} [H]
\small
\centering
\begin{tabular}{| c | c |}
\hline \bf Model Type & \bf Accuracy (\%) \\ \hline
CBOW (100) & 45 \\
CBOW (300) & 50 \\
CBOW (500) & 61 \\
CBOW (750) & 62 \\
CBOW (1000) & 65 \\
\hline
\end{tabular}
\caption{\label{different_cbow} Sentence length accuracy for different CBOW representation sizes.}
\end{table}

\mycomment{Table~\ref{different_cbow} summarize the results for CBOW with different embedding sizes. It is interesting to note that when the embedding size gets larger the better it can classify the sentence length.}

\begin{table} [H]
\small
\centering
\begin{tabular}{| c | c |}
\hline \bf Model Type & \bf Accuracy (\%) \\ \hline
CBOW (100) & 37\\
CBOW (300) & 50\\
CBOW (500) & 57\\
CBOW (750) & 60\\
CBOW (1000) & 61\\
\hline
\end{tabular}
\caption{\label{different_cbow_no_lang} Sentence length accuracy for different CBOW representation sizes on synthetic sentences.}
\end{table}

To address the question we raised regarding the success of CBOW at this test we randomly sampled words from the dictionary and created synthetic sentences. Than, we repeated the length experiment using the same configuration.
It seems from Table~\ref{different_cbow_no_lang} that the accuracy slightly decreased from the one with real sentences. \mycomment{INSERT EINAT INSIGHT ABOUT THAT}.

%%% LANGUAGE %%%
\subsection{Is It About Language?}

Some of the results from the previous sub-sections, especially CBOW results, raise the following question, is it about the language? In other words, does the high accuracy rates in tasks like predicting words order or sentence length were effected mainly by language structure or language statistics. In order to separate language properties from the encoding algorithm we permute the sentences, generate new representations based on the original trained models and execute the content, length and order tests. While sentence representation is the same for CBOW also after permutation it completely changes when generated by the the encoder-decoder, this is the reason we decided to execute all three tests. It can be seen from Table~\ref{permute_sent} that language properties have a minor effect on the encoded sentences generated by the encoder-decoder. Information about words order exists also after words permutation. Another interesting property to note is the sentence length accuracy, LSTM of size 500 and 750 got benefit from the permutation, it helped them to better classify sentence length.

\begin{table*}[htbp]
\small
\centering
\begin{tabular}{| P{1.3in} | P{1.3in} | P{1.3in} | P{1.3in} |}
\hline
\bf Model Type & \bf Sentence Length (\%) & \bf Random Word (\%) & \bf Order of Words (\%)\\ \hline
LSTM (100) & 46 & 70 & 73\\
LSTM (300) & 80 & 76 & 82\\
LSTM (500) & 89 & 77 & 85\\
LSTM (750) & 93 & 80 & 85\\
LSTM (1000) & 85 & 72 & 90\\
CBOW (100) & 45 & 83 & 50\\
CBOW (300) & 50 & 86 & 50\\
CBOW (500) & 61 & 60 & 50\\
CBOW (750) & 62 & 59 & 50\\
CBOW (1000) & 65 & 60 & 50\\
\hline
\end{tabular}
\caption{\label{permute_sent} Permute sentences results.}
\end{table*}

%%% GENERALIZATION %%%
\subsection{Generalization}
In the word content test our goal is to qualify the relation between word and sentence representations. This test will classify whether a word did or did not appear in a given sentence. In real life tasks we sometimes need to find relations not with the exact word, but with some semantically close word. For example, in paraphrase classification we need to find relations between two sentences that do not contain the exact words. Hence, we extend the word content test to include some generalization properties. We create 15 different tests that examine how well a model can find relations between a sentence and a word that is close to some random word from it. Following the word content architecture, we randomly picked a word, $w$, from each sentence and compute its 1st, 10th, 50th, 100th and 500th closest words (we use the Euclidian distance between words representations as our metric), denote $w_{1}, w_{10}, w_{50}, w_{100}, w_{500}$. Than, for each pair of those words, we generates a different test the same way as in the word content. For example, in the $w_{10} vs. w_{50}$ test, we concatenate to the sentence representation of the 10th closest word to the sentence representation and set this as positive example, for negative example we use the representation of the 50th closest word. That way, we can qualify the ability of  a model to generate representations that can generalize well. Results are summarized in Table~\ref{random_k}.
\mycomment{ADD SOME INSIGHT ABOUT THE RESULTS}

\begin{table*}[htbp]
\small
\small
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{| c | c | c | c | c | c | c | c | c |}
\hline
\bf Model Type & \bf $w vs. w_{1}$ & \bf $w vs. w_{10}$ & \bf $w vs. w_{50}$ & \bf $w vs. w_{100}$ & \bf $w vs. w_{500}$ & \bf $w_{1} vs. w_{10}$ & \bf $w_{1} vs. w_{50}$ & \bf $w_{1} vs. w_{100}$\\ 
\hline
LSTM (1000) & 96 & 95 & 95 & 94 & 93 & 81 & 84 & 85 \\
LSTM (750) & 77 & 82 & 85 & 86 & 88 & 75 & 79 & 80 \\
LSTM (500) & 74 & 79 & 82 & 84 & 86 & 72 & 75 & 77 \\
\hline
CBOW (300) & 82 & 87 & 92 & 94 & 97 & 80 & 85 & 87 \\
CBOW (100) & 72 & 78 & 82 & 85 & 92 & 72 & 77 & 80 \\
\hline
\\
\hline
& \bf $w_{1} vs. w_{500}$  & \bf $w_{10} vs. w_{50}$ & \bf $w_{10} vs. w_{100}$ & \bf \bf $w_{10} vs. w_{500}$ & \bf $w_{50} vs. w_{100}$ & \bf $w_{50} vs. w_{500}$ & \bf $w_{100} vs. w_{500}$ & \bf - \\ 
\hline
LSTM (1000) & 89 & 82 & 83 & 87 & 83 & 85 & 85 & - \\
LSTM (750) & 83 & 76 & 77 & 80 & 75 & 78 & 76 & - \\
LSTM (500) & 80 & 71 & 73 & 77 & 69 & 73 & 72 & - \\
\hline
CBOW (300) & 92 & 71 & 73 & 78 & 61 & 65 & 60 & - \\
CBOW (100) & 90 & 72 & 76 & 87 & 68 & 78 & 71 & - \\
\hline
\end{tabular}}
\caption{\label{random_k} Generalization experiments for CBOW with size 100 and 300 and encoder-Decoder with size 500, 750 and 1000. All the results are in percentage.}
\end{table*}

%%%Operational stuff %%%
\subsection{Operational stuff}
Figure xxx shows å comparison of encoder-decoder models with two loss functions: negative log-likelihood and cosine similarity.  The \hl{regression} model has a comparable performance to the standard model, despite having much fewer parameters and better run time. \hl{Einat: do you have some numbers to support this? Also, add the comparable numbers from the standard log-likelihood model so it's easier to compare.}
%Our implementation of the encoder-decoder model depends on the size of the dictionary. It includes a word embedding layer which maps each word to its representation and a softmax layer which calculates the probability distribution of the predicted word given its representation as calculated by the LSTM. The size of these layers is the size of the dictionary, 50K in our models, times the LSTM dimension. Therefore, in order to reduce the size of the model we remove the softmax layer and replace the negative log-likelihood loss function by cosine similarity loss function. In this case the word representation of the predicted word is compared with the word representation of the required word instead of comparing the indexes. We call this model a regression model. Figure xxx present the performance of this model on the various tests. It is possible to see that the regression model has comparative results.

\begin{table} [H]
\small
\centering
\begin{tabular}{| c | c | c |}
\hline \bf Sentence Length & \bf Random Word & \bf Order of Words \\ \hline
91\% & 75\% & 90\%\\
\hline
\end{tabular}
\caption{\label{regr_results} All tests results for the encoder-decoder with representation size 1000 trained to predict the words representations.}
\end{table}

%%% Semantic test %%%
\subsection{Extension of the Content Experiments}
In the content experiment we defined a binary classification task that could be too easy to learn. We would like to challenge the model by more difficult task. Therefor we defined a task that given the sentence representation try to predict the kth word in the sentence. For example, when k=2 the network should learn to predict the second word in the sentences when it has its sentence representation. Note that this is a multi-label classification task when the number of labels is the size of the dictionary, 50K in our case. We noticed that in all the models there is not enough information to predict words that are not in the beginning of the sentence and some models have the ability to predict the first words in the sentences. Table xxx presents those results. CBOW and BI-LSTM have very poor results therefore they do not appear in the table. It is possible to see in the table that LSTM model size 500 outperforms all the rests of the model. In addition the regression model which its size is 1000 gives better results than the basic model in the same size.  We conclude that the sentence representation created by the encoder-decoder models have mostly information regarding the first word in the sentence and as you move away from the beginning of the sentence that information reduces significantly.

%%% Semantic test %%%
\subsection{Semantic test}
In order to give a broader view on the performance of the sentences embedding models we decided to include in our analysis one natural language processing popular task with semantic aspects. We chose to compare the performance of the models on task of natural language inference using the Stanford Natural Language Inference (SNLI) corpus \citep{bowman2015}. 
We defined a simple configuration for the comparison, did not try to look for the best configuration to achieve the state-of-the-art results. The architecture we use is as follow: the encoder part of the encoder-decoder model is duplicated in order to create a parallel encoding units for the premise and for the hypothesis. The output vector of the encoders are concatenated and delivered to a fully connected layer with tanh activation function. The last layer of the model is a softmax layer which gives classification of three labels: entailment, contradiction, and neutral. We add after the LSTM a dropout unit with rate of 0.5 and optimize our objective using AdaGrad, a variation of Stochastic Gradient Descent. Table xxx present the train and test accuracy of the various model. The model that reaches the best results is the LSTM of size 500. We can see here again the discrepancy between the quality measures (BLEU) which gives the LSTM of size 1000 the highest score and the results on a specific task which in this case LSTM of size500 hat reaches the best accuracy.

\begin{table} [H]
\small
\centering
\begin{tabular}{| c | c | c |}
\hline \bf Representation Size & \bf Test (\%acc) & \bf Train (\%acc) \\ \hline
1000 & 69.3 & 77.74 \\
750 & 71.4 & 79.1 \\
500 & 73.1 & 77.8\\
300 & 71 & 77.5\\
100 & 68.4 & 73 \\
\hline
\end{tabular}
\caption{\label{natural_language_inference  } Natural language inference task.}
\end{table}


%% SUMMARY %%


